Evaluating Zero-Shot GPT-4V Performance on 3D Visual Question Answering Benchmarks

As interest in "reformulating" the 3D Visual Question Answering (VQA) problem in the context of foundation models grows, it is imperative to assess how these new paradigms influence existing closed-vocabulary datasets. In this case study, we evaluate the zero-shot performance of foundational models (GPT-4 Vision and GPT-4) on well-established 3D VQA benchmarks, namely 3D-VQA and ScanQA. We provide an investigation to contextualize the performance of GPT-based agents relative to traditional modeling approaches. We find that GPT-based agents without any fine-tuning perform on par with the closed vocabulary approaches. Our findings corroborate recent results that "blind" models establish a surprisingly strong baseline in closed-vocabulary settings. We demonstrate that agents benefit significantly from scene-specific vocabulary via in-context textual grounding. By presenting a preliminary comparison with previous baselines, we hope to inform the community's ongoing efforts to refine multi-modal 3D benchmarks.

==> sec/4_methodology.tex <==
\section{Methodology Details}
\label{sec:methodology}

\textbf{Orchestrator.} Blah blah

\textbf{Prompting.}

\begin{tcolorbox}[title=Reference Caption, colback=gray!20, colframe=gray!75, rounded corners, sharp corners=northeast, sharp corners=southwest]
\footnotesize
\texttt{\textbf{Reference Q:} Use the YOLO detector to detect fishing vessels in xview3 images around Ancona. Plot them on the map.\\
\textbf{Paraphrased Q:} Use RetinaNet to find yacht detections in xview1 images around Barbados, and show them on the map.\\
\textbf{Perturbed Q:} Use NoNet to find Zeppelins in images around the mythical city of Atlantis.}
\end{tcolorbox}

\textbf{Batched prompting.} 

\begin{tcolorbox}[title=Reference Caption, colback=gray!20, colframe=gray!75, rounded corners, sharp corners=northeast, sharp corners=southwest]
\footnotesize
\texttt{\textbf{Reference Q:} Use the YOLO detector to detect fishing vessels in xview3 images around Ancona. Plot them on the map.\\
\textbf{Paraphrased Q:} Use RetinaNet to find yacht detections in xview1 images around Barbados, and show them on the map.\\
\textbf{Perturbed Q:} Use NoNet to find Zeppelins in images around the mythical city of Atlantis.}
\end{tcolorbox}

\textbf{Force-a-guess.} Blah blah


